Lessons from the trenches on evaluating machine-learning systems in materials science

Measurements are fundamental to knowledge creation in science, enabling consistent sharing of findings and serving as the foundation for scientific discovery. As machine learning systems increasingly transform scientific fields, the question of how to effectively evaluate these systems becomes crucial for ensuring reliable progress. In this review, we examine the current state and future directions of evaluation frameworks for machine learning in science. We organize the review around a broadly applicable framework for evaluating machine learning systems through the lens of statistical measurement theory, using materials science as our primary context for examples and case studies. We identify key challenges common across machine learning evaluation such as construct validity, data quality issues, metric design limitations, and benchmark maintenance problems that can lead to phantom progress when evaluation frameworks fail to capture real-world performance needs. By examining both traditional benchmarks and emerging evaluation approaches, we demonstrate how evaluation choices fundamentally shape not only our measurements but also research priorities and scientific progress. These findings reveal the critical need for transparency in evaluation design and reporting, leading us to propose evaluation cards as a structured approach to documenting measurement choices and limitations. Our work highlights the importance of developing a more diverse toolbox of evaluation techniques for machine learning in materials science, while offering insights that can inform evaluation practices in other scientific domains where similar challenges exist.

==> reporting_card.tex <==
# Benchmark Reporting Card

## Estimand Definition
### Target Measurement
- Primary quantity of interest: [What fundamental property/capability are we trying to measure?]
- Scientific relevance: [How does this connect to real-world applications?]
- Scope limitations: [Explicit boundaries of what is being measured]

### Data Characteristics
- Population definition: [What is the target population?]
- Sampling strategy: [How representative is the data?]
- Label source: [Origin and quality of ground truth]
- Known biases: [Documented limitations in coverage]

### Metric Definition
- Primary metrics: [Mathematical definition]
- Theoretical bounds: [Expected range and limitations]
- Real-world correlation: [Evidence of construct validity]

## Estimator Design
### Evaluation Protocol
- Split strategy: [How data is partitioned]
- Cross-validation approach: [If applicable]
- Uncertainty quantification method: [How confidence intervals are computed]

### Implementation
- Reference implementation: [Link to code]
- Computational requirements: [Hardware/software needs]
- Reproducibility protocol: [Steps to reproduce results]

## Estimate Reporting
### Performance Metrics
- Aggregate scores: [Overall performance]
- Uncertainty bounds: [Confidence intervals]
- Disaggregated analysis: [Performance across subgroups]

### Limitations
- Known failure modes: [Documented weaknesses]
- Generalization bounds: [Statistical guarantees if available]
- Environmental impact: [Computational cost]

### Version Control
- Benchmark version: [Version number]
- Change log: [Major updates]
- Legacy compatibility: [Backward compatibility notes]

